Ruppeiner theory of black hole thermodynamics

The Ruppeiner metric as determined by the Hessian of the Gibbs surface provides a geometric description of thermodynamic systems in equilibrium. An interesting example is a black hole in equilibrium with its own Hawking radiation. In this article, we present results from the Ruppeiner study of various black hole families from different gravity theories e.g. 2D dilaton gravity, BTZ, general relativity and higher-dimensional Einstein-Maxwell gravity.

==> macros.tex <==
\newcommand{\Ix}[1]{#1\index{#1}}

\newcommand{\chf}{\,{_1{\cal F}_1}} % confluent hypergeometric function

%% for Index entries use \Ix{keyword} instead of ``keyword'' in text!

\newcommand{\beqs}{\begin{equation*}}
\newcommand{\beq}{\begin{equation}}

\newcommand{\eeqs}{\end{equation*}}
\newcommand{\eeq}{\end{equation}}

\newcommand{\beqas}{\begin{eqnarray*}}
\newcommand{\beqa}{\begin{eqnarray}}

\newcommand{\eeqas}{\end{eqnarray*}}
\newcommand{\eeqa}{\end{eqnarray}}

\newcommand{\seq}[5]{\newline 
\parbox{#1}{\begin{eqnarray*} #2 \end{eqnarray*}} \hfill
\parbox{#3}{\begin{eqnarray*} #4 \end{eqnarray*}} \hfill
\parbox{1cm}{\begin{equation} \label{#5} \end{equation}} 
\newline}

%% Syntax example: \seq{2cm}{equationarray1}{3cm}{equationarray2}{superlabel99}

\newcommand{\eqs}[1]{\begin{equation} #1 \end{equation}}

%% equations sine label

\newcommand{\eqas}[1]{\begin{eqnarray} #1 \end{eqnarray}}

%% equation-arrays sine label

\newcommand{\eq}[2]{\begin{equation} #1 \label{#2} \end{equation}}

%% equations which are labeled

\newcommand{\eqa}[2]{\begin{eqnarray} #1 \label{#2} \end{eqnarray}}

%% equation arrays which have one label in the last line

\newcommand{\meq}[2]{\begin{multline} #1 \label{#2} \end{multline}}

%% for multi-line equations...

\newcommand{\eps}{\varepsilon}
\newcommand{\al}{\alpha}
\newcommand{\be}{\beta}
\newcommand{\ga}{\gamma}
\newcommand{\de}{\delta}
\newcommand{\om}{\omega}
\newcommand{\ka}{\kappa}
\newcommand{\la}{\lambda}
\newcommand{\si}{\sigma}
\newcommand{\Eps}{\Varepsilon}
\newcommand{\Al}{\Alpha}
\newcommand{\Be}{\Beta}
\newcommand{\Ga}{\Gamma}
\newcommand{\De}{\Delta}
\newcommand{\Om}{\Omega}
\newcommand{\Ka}{\Kappa}
\newcommand{\La}{\Lambda}
\newcommand{\Si}{\Sigma}
\newcommand{\Th}{\Theta}

%% greek letters

\newcommand{\qb}{q_{\bot}}
\newcommand{\pb}{p_{\bot}}

\newcommand{\blist}{\begin{itemize}}

\newcommand{\elist}{\end{itemize}}

\newcommand{\dummy}[1]{#1}

%% just to mark a (text-)position in the buffer with ``dummy'' - e.g. when some
%% English expression is not know

\providecommand{\href}[2]{#2}
\newcommand{\URL}[1]{{\href{#1}{{\tt{\small{#1}}}}}}

\newcommand{\myURL}{\href{http://stop.itp.tuwien.ac.at/~grumil/projects/myself/thesis/s4.nb}{{\tt{\small{http://stop.itp.tuwien.ac.at/$\sim$grumil/projects/myself/thesis/s4.nb}}}}}

%% for hyperreferences

\newcommand{\chapquote}[2]{{\it #1}\begin{flushright}#2\end{flushright}}

%% for quotes right after a chapter

\newcommand{\twod}{$2D$}

%% further twodsided extension of \clearpage

\newcommand{\clearemptydoublepage}{\newpage{\pagestyle{empty}\cleardoublepage}}
\newcommand{\clearplaindoublepage}{\newpage{\pagestyle{plain}\cleardoublepage}}

\newcommand{\newtext}[1]{{\bf #1}}

\newcommand{\unity}{1\hspace{-0.243em}\text{l}}

% \newcommand{\scri}{\mathcal{I}}

 %%% definition of scri
\DeclareFontFamily{OT1}{rsfs}{}
\DeclareFontShape{OT1}{rsfs}{m}{n}{ <-7> rsfs5 <7-10> rsfs7 <10->rsfs10}{} 
\DeclareMathAlphabet{\mycal}{OT1}{rsfs}{m}{n}
\newcommand{\scri}{{\mycal I}}

